An Instrument Error Budget for Space-Based Absolute Flux Measurements of the Sky Synchrotron Spectrum Below 20 MHz

This work describes the instrumental error budget for space-based measurements of the absolute flux of the sky synchrotron spectrum at frequencies below the ionospheric cutoff (<20 MHz). We focus on an architecture using electrically short dipoles onboard a small satellite. The error budget combines the contributions of the dipole dimensions, plasma noise, stray capacitance, and front-end amplifier input impedance. We treat the errors using both a Monte Carlo error propagation model and an analytical method. This error budget can be applied to a variety of experiments and used to ultimately improve the sensing capabilities of space-based electrically short dipole instruments. The impact of individual uncertainty components, particularly stray capacitance, is explored in more detail.

==> Appendices/Analytical_Propagation.tex <==
Analytical uncertainty propagation was done for comparison to the Monte Carlo technique. This involved describing the uncertainty of the parameters using partial derivatives and combining appropriately. This appendix describes the formalism and steps to achieve the analytical uncertainty result.

The antenna capacitance is given by:
\begin{equation}
C_{a}=\frac{2 \pi \epsilon_{0} L}{\ln \left(\frac{L}{a}\right)-1}
\end{equation}
The uncertainty is given by:
\begin{equation}
\Delta C_{a}^{2}=\Delta L^{2}\left|\frac{\partial C_{a}}{\partial L}\right|^{2}+\Delta a^{2}\left|\frac{\partial C_{a}}{\partial a}\right|^{2}
\end{equation}
Taking the derivative with respect to $L$ and $d$ :
\begin{equation}
\begin{gathered}
\frac{\partial C_{a}}{\partial L}=\frac{2 \pi \epsilon_{0}\left[\ln \left(\frac{L}{a}\right)-2\right]}{[\ln \left(\frac{L}{a}\right)-1]^{2}} \\
\frac{\partial C_{a}}{\partial a}=\frac{2 \pi \epsilon_{0} L}{a\left[\ln \left(\frac{L}{a}\right)-1\right]^{2}}
\end{gathered}
\end{equation}
Then
\begin{equation}
\Delta C_{a}^{2}=\left(\Delta L \frac{2 \pi \epsilon_{0}\left[\ln \left(\frac{L}{a}\right)-2\right]}{\left[\ln \left(\frac{L}{a}\right)-1\right]^{2}}\right)^{2}+\left(\Delta a \frac{2 \pi \epsilon_{0} L}{a\left[\ln \left(\frac{L}{a}\right)-1\right]^{2}}\right)^{2}
\end{equation}
Dividing by the expression for $C_{a}$ gives the relative uncertainty:
\begin{equation}
\begin{gathered}
\left(\frac{\Delta C_{a}}{C_{a}}\right)^{2}=\left(\Delta L \frac{\left[\ln \left(\frac{L}{a}\right)-2\right]}{L\left[\ln \left(\frac{L}{a}\right)-1\right]}\right)^{2}+\left(\Delta a \frac{1}{a\left[\ln \left(\frac{L}{a}\right)-1\right]}\right)^{2} \\
\left(\frac{\Delta C_{a}}{C_{a}}\right)^{2}=\left(\frac{\Delta L}{L} \frac{\ln \left(\frac{L}{a}\right)-2}{\ln \left(\frac{L}{a}\right)-1}\right)^{2}+\left(\frac{\Delta a}{a} \frac{1}{\ln \left(\frac{L}{a}\right)-1}\right)^{2}
\end{gathered}
\end{equation}

\noindent In the limit of small antenna resistance, and at low frequencies where $X\simeq -1/(2\pi f C )$, a simplified version of the voltage divider is given by:
\begin{equation}
\Gamma=\left(1+\frac{C_{s}}{C_{a}}\right)^{-2}
\end{equation}
The uncertainty is given by:
\begin{equation}
\Delta \Gamma^{2}=\Delta C_{s}^{2}\left|\frac{\partial \Gamma}{\partial C_{s}}\right|^{2}+\Delta C_{a}^{2}\left|\frac{\partial \Gamma}{\partial C_{a}}\right|^{2}
\end{equation}
Taking the derivative with respect to $C_{s}$ and $C_{a}$ :
\begin{equation}
\begin{gathered}
\frac{\partial \Gamma}{\partial C_{s}}=-\frac{2}{C_{a}}\left(1+\frac{C_{s}}{C_{a}}\right)^{-3} \\
\frac{\partial \Gamma}{\partial C_{a}}=-2 \frac{C_{s}}{C_{a}}\left(1+\frac{C_{S}}{C_{a}}\right)^{-3}
\end{gathered}
\end{equation}
Then
\begin{equation}
\Delta \Gamma^{2}=\left(\Delta C_{s} \frac{2}{C_{a}}\left(1+\frac{C_{s}}{C_{a}}\right)^{-3}\right)^{2}+\left(\Delta C_{a} 2 \frac{C_{s}}{C_{a}^{2}}\left(1+\frac{C_{s}}{C_{a}}\right)^{-3}\right)^{2}
\end{equation}
Dividing by the expression for $\Gamma$ gives the relative uncertainty:
\begin{equation}
\begin{aligned}
&\left(\frac{\Delta \Gamma}{\Gamma}\right)^{2}=\left(\Delta C_{s} \frac{2}{C_{a}}\left(1+\frac{C_{s}}{C_{a}}\right)^{-1}\right)^{2}+\left(\Delta C_{a} 2 \frac{C_{s}}{C_{a}^{2}}\left(1+\frac{C_{s}}{C_{a}}\right)^{-1}\right)^{2} \\
&\left(\frac{\Delta \Gamma}{\Gamma}\right)^{2}=\left(\frac{\Delta C_{s}}{C_{s}} 2 \frac{C_{s}}{C_{a}}\left(1+\frac{C_{s}}{C_{a}}\right)^{-1}\right)^{2}+\left(\frac{\Delta C_{a}}{C_{a}} 2 \frac{C_{s}}{C_{a}}\left(1+\frac{C_{s}}{C_{a}}\right)^{-1}\right)^{2}
\end{aligned}
\end{equation}

\noindent The voltage to flux term is given by:
\begin{equation}
\chi=x \frac{L_{m}}{\left(1+\frac{C_{S}}{C_{a}}\right)^{2}}
\end{equation}
Where $x$ is the constant $80\pi\,\Omega$.
The uncertainty is given by:
\begin{equation}
\Delta \chi^{2}=\Delta L_{m}^{2}\left|\frac{\partial \chi}{\partial L_{m}}\right|^{2}+\Delta C_{s}^{2}\left|\frac{\partial \chi}{\partial C_{s}}\right|^{2}+\Delta C_{a}^{2}\left|\frac{\partial \chi}{\partial C_{a}}\right|^{2}
\end{equation}
Taking the derivative with respect to $L_{m}, C_{s}$ and $C_{a}$ :
\begin{equation}
\begin{aligned}
\frac{\partial \chi}{\partial L} &=\frac{x}{\left(1+\frac{C_{s}}{C_{a}}\right)^{2}} \\
\frac{\partial \chi}{\partial C_{s}} &=\frac{2 C_{a}^{2} L x}{\left(C_{a}+C_{s}\right)^{3}} \\
\frac{\partial \chi}{\partial C_{a}} &=\frac{2 C_{a} C_{s} L x}{\left(C_{a}+C_{s}\right)^{3}}
\end{aligned}
\end{equation}
Then
\begin{equation}
\Delta \chi^{2}=\left(\Delta L_{m} \frac{x}{\left(1+\frac{C_{s}}{C_{a}}\right)^{2}}\right)^{2}+\left(\Delta C_{s} \frac{2 L x}{C_{a}\left(1+\frac{C_{S}}{C_{a}}\right)^{3}}\right)^{2}+\left(\Delta C_{a} \frac{2 C_{s} L x}{C_{a}^{2}\left(1+\frac{C_{s}}{C_{a}}\right)^{3}}\right)^{2}
\end{equation}
Dividing by the expression for $\chi$ gives the relative uncertainty:
\begin{equation}
\begin{gathered}
\left(\frac{\Delta \chi}{\chi}\right)^{2}=\Delta L_{m}^{2}+\left(\Delta C_{s} \frac{2\left(1+\frac{C_{s}}{C_{a}}\right)^{2}}{C_{a}\left(1+\frac{C_{s}}{C_{a}}\right)^{3}}\right)^{2}+\left(\Delta C_{a} \frac{2 C_{s}\left(1+\frac{C_{s}}{C_{a}}\right)^{2}}{C_{a}^{2}\left(1+\frac{C_{s}}{C_{a}}\right)^{3}}\right)^{2} \end{gathered}
\end{equation}
\begin{equation}\label{eq.conversion_uncertainty}
\begin{gathered}
\left(\frac{\Delta \chi}{\chi}\right)^{2}=\left(L_{m} \frac{\Delta L_{m}}{L_{m}}\right)^{2}+\left(\frac{\Delta C_{s}}{C_{s}} \frac{C_{s}}{C_{a}} \frac{2}{\left(1+\frac{C_{s}}{C_{a}}\right)}\right)^{2}+\left(\frac{\Delta C_{a}}{C_{a}} \frac{C_{s}}{C_{a}} \frac{2}{\left(1+\frac{C_{s}}{C_{a}}\right)}\right)^{2}
\end{gathered}
\end{equation}

The plasma voltage at the antenna is given by:
\begin{equation}
U_{p}=5 \times 10^{-5} \frac{n_{e} T_{e}}{f^{3} L_{m}} \Gamma
\end{equation}
Since there are only multiplicative terms in the expression for $U_{p}$, the relative uncertainty is just the relative uncertainty of the components added in quadrature:
\begin{equation}
\left(\frac{\Delta U_{p}}{U_{p}}\right)^{2}=\left(\frac{\Delta L_{m}}{L_{m}}\right)^{2}+\left(\frac{\Delta n_{e}}{n_{e}}\right)^{2}+\left(\frac{\Delta T_{e}}{T_{e}}\right)^{2}+\left(\frac{\Delta \Gamma}{\Gamma}\right)^{2}
\end{equation}

The voltage and uncertainty from the amplifier is given by 
\begin{equation}
U_a = U_{V} + U_{I} + +U_{J}
\end{equation}
\begin{equation}
\Delta U_{a}=\sqrt{\Delta U_{V}^{2}+\Delta U_{I}^{2}+\Delta U_{j}^{2}}
\end{equation}

The operational amplifier voltage noise, $U_V$, is simply $V_n^2$, where $V_n$ is the voltage noise density specification of the component used. The operational amplifier current noise, $U_{I}$, is $(I_n\times |Z_{eq}|)^2$, where $I_n$ is the current noise density specification of the component used, and $Z_{eq}$ is the impedance of the circuit looking out from the input terminals of the amplifier. Finally, the Johnson–Nyquist thermal noise is given by $U_{J} = 4k_B T_0 R_T$, where $k_B$ is the Boltzmann constant, $T_0$ is the temperature of the system, and $R_T$ is the total resistance.


% low compared to other components and constant with so the total assumed value is taken to be that found by the Monte Carlo estimate of $1.3 \%$. The mean of the receiver noise is constant at $2.17 \times 10^{-17} V^{2} H z^{-1}$.
The received voltage from the galactic flux is given by:
\begin{equation}
U_{g}=U_{m}-U_{p}-U_{a}
\end{equation}
The effective Galactic voltage uncertainty is thus given by
\begin{equation}
\Delta U_{g}=\sqrt{\Delta U_{m}^{2}+\Delta U_{p}^{2}+\Delta U_{a}^{2}}
\end{equation}
We need to use absolute uncertainties, because although the relative uncertainties for each of these expressions are constant, the actual values vary with frequency.
\begin{equation}\label{eg.ug_uncertainty}
\Delta U_{g}^{2}=\left(\frac{\Delta U_{m}}{U_{m}} U_{m}\right)^{2}+\left(\frac{\Delta U_{p}}{U_{p}} U_{p}\right)^{2}+\left(\frac{\Delta U_{a}}{U_{a}} U_{a}\right)^{2}
\end{equation}
where $U_M$ is described simply by the calibration components of uncertainty added in quadrature.
% Using the values and expressions found above:
% $$
% \Delta U_{g}=\sqrt{\left((0.183)\left(5 \times 10^{-5} \frac{n_{e} T_{e}}{f^{3} L_{m}} \Gamma\right)\right)^{2}-\left((0.013)\left(2.17 \times 10^{-17}\right)\right)^{2}}
% $$
Finally, the predicted flux is given by
\begin{equation}
S_{g}=\frac{U_{g}}{\chi}
\end{equation}
The relative uncertainty is just the relative uncertainty of the components added in quadrature, which have already been derived above in Equations~\ref{eg.ug_uncertainty} and~\ref{eq.conversion_uncertainty}:
\begin{equation}
\begin{gathered}
\frac{\Delta S_{g}}{S_{g}}=\sqrt{\left(\frac{\Delta U_{g}}{U_{g}}\right)^{2}+\left(\frac{\Delta \chi}{\chi}\right)^{2}} \end{gathered}
\end{equation}


==> Appendices/Finite_Resistance_and_Reactance.tex <==
The NEC2 simulations and the electrically short dipole approximations of the radiation resistance and the antenna reactance is presented in Figure~\ref{fig:resistance_vs_length} and~\ref{fig:reactance_vs_length}. The disparity between approximation and the simulation can be partially resolved using analytical expressions for a finite dipole given in~\cite{balanis-textbook}:

\begin{multline}
R_{rad} = \frac{\eta}{2\pi \sin^{2}(kL/2)} \biggl\{C + \ln{(kL)} - C_i(kL)
+ \frac{1}{2}\sin{(kL)} \left[ S_i(2kL) - 2S_i(kL)\right] \\
+ \frac{1}{2}\cos{(kL)} \left[ C + \ln{(kL/2)} + C_i(2kL) - 2C_i(kL)\right]\biggl\}
\end{multline}
And
\begin{multline}
X_a = \frac{\eta}{4\pi \sin^{2}(kL/2)} \biggl\{2S_i(kL) + \cos{(kL)}[2S_i(kL)-S_i(2kL)] \\
- \sin{(kL)} \left[ 2C_i(kL) - C_i(2kL) - C_i(\frac{2kr^2}{L})\right]\biggl\}
\end{multline}

where $\eta$ is the intrinsic impedance of the medium, $L$ is the full length, $k$ is the wave number, $C$ is Euler's constant, and $r$ is the radius. $C_i$ and $S_i$ are the cosine and sine integrals given by
\begin{equation}
C_i = -\int^{\infty}_{x} \frac{\cos y}{y} dy = \int^{x}_{\infty} \frac{\cos y}{y}
\end{equation}
And
\begin{equation}
S_i = \int^{x}_{0} \frac{\sin y}{y} dy
\end{equation}


Recreations of Figure~\ref{fig:resistance_vs_length} and~\ref{fig:reactance_vs_length} are given below, with the finite dipole equations used instead of the electrically short approximations.

\begin{figure*}[ht]
    \centering
    \includegraphics[width=.47\textwidth]{Appendices/resistance_vs_length_exact.pdf}\hspace{.2 in}
    \includegraphics[width=.47\textwidth]{Appendices/resistance_vs_length_percent_difference_exact.pdf}
    % \\[\smallskipamount]
        \caption{The finite equation version of Figure~\ref{fig:resistance_vs_length}. Left: The antenna radiative resistance versus full dipole length at five different frequencies. The NEC2 simulation shown by the solid line and the dotted line shows the finite dipole analytical expression. Right: The percent relative difference between the NEC2 simulation results and the analytical expression.}
    \label{fig:resistance_vs_length_exact}
\end{figure*}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=.47\textwidth]{Appendices/reactance_vs_length_exact.pdf}\hspace{.2 in}
    \includegraphics[width=.47\textwidth]{Appendices/reactance_vs_length_percent_difference_exact.pdf}
    % \\[\smallskipamount]
        \caption{The finite equation version of Figure~\ref{fig:reactance_vs_length}. Left: The antenna reactance versus full dipole length at five different frequencies. The NEC2 simulation shown by the solid line and the dotted line shows the finite dipole analytical expression. Right: The percent absolute relative difference between the NEC2 simulation results and the analytical expression.}
    \label{fig:reactance_vs_length_exact}
\end{figure*}


The percent difference between the short dipole approximation and the finite dipole equation is given in Figure~\ref{fig:finite_compare_to_esd}.

\begin{figure*}[ht]
    \centering
    \includegraphics[width=.47\textwidth]{Appendices/resistance_vs_length_esd_compare_exact.pdf}\hspace{.2 in}
    \includegraphics[width=.47\textwidth]{Appendices/reactance_vs_length_esd_compare_exact.pdf}
    % \\[\smallskipamount]
        \caption{Percent difference between the electrically short dipole and the finite dipole equations for the radiative resistance (left) and the antenna reactance (right).}
    \label{fig:finite_compare_to_esd}
\end{figure*}


==> Appendices/Flux_to_Voltage_Conversion.tex <==
This appendix describes the derivation of the flux to voltage conversion.  

% % [Balanis Eq. 2-93]
% % [Stutzman Eq. 4-1]
% % [Krauss88 Eq 2-19-1]
% where $V_{oc}$ is the open circuit voltage and $E_i$ is the incident electric field. 

The effective area, $A_e$, (also called effective or equivalent aperture), is defined as the ratio of the available power at the terminals of a receiving antenna when a wave impinges on it:
\begin{equation}\label{eq:Ae1}
A_e = \frac{P_T}{S} = \frac{|I_T|^2 R_t/2}{S}
\end{equation}
% [Balanis Eq. 2-94]
% [Stutzman Eq. 4-6]
% [Kraus50 Eq. 3-9]
% [Krauss88 Eq. 2-13-8]
where $P_{T}$ is the power delivered to the load (in W) and $S$ is the power density of the incident wave (in W/m$^2$). The effective area can be calculated in a number of different ways. 
% Note look more into Balanis Eq. 2-95.
In relation to the directivity, $D$, the effective area is given by
\begin{equation}\label{eq:Ae2}
A_{e} = \frac{\lambda^2}{4\pi} D
\end{equation}
% [Balanis Eq. 2-111]
% [Stutzman Eq. 4-23]
% [Kraus50 Eq. 3-47]
% [Krauss88 Eq. 2-22-10]
% and
In terms of the impedance of free space, $Z_0$, the effective length, $\ell$, and the radiative resistance, the effective area is given by:
\begin{equation}\label{eq:Ae3}
A_e = \frac{\ell^2 Z_0}{4 R_r} 
\end{equation}
% [Kraus50 Eq. 3-11]
% [Krauss88 Eq. 2-19-6]

Equating Eq.~\ref{eq:Ae2} and~\ref{eq:Ae3} and solving for $\ell^2$:

\begin{equation}\label{eq:ell}
\ell^2 = \frac{\lambda^2 D}{4\pi} \frac{4 R_r}{Z_0}
\end{equation}

% Also note: source brightness is related to E by: $B = E^2/Z_0$ or $E^2 = B Z_0$. 

Consider, the voltage induced on the open circuit terminals when a wave impinges on it is related to the effective length, $\ell$,  and the voltage divider, $\Gamma$:
\begin{equation}\label{eq:voc}
V_{oc} = E_i \ell \Gamma
\end{equation}

The voltage squared produced by an E field from an infinitesimal solid angle, $d\Omega$, is then given by 
\begin{equation}\label{eq:voc_squared}
d(V_{oc}^2) = E_i^2 \ell^2 \Gamma^2 d\Omega
\end{equation}

Substitute $E^2$ in terms of brightness ($E^2 = B Z_0$) and the expression for effective length from Eq.~\ref{eq:ell}:
$$d(V_{oc}^2) = B Z_0 \left(\frac{\lambda^2 D(\Omega)}{4\pi} \frac{4 R_r}{Z_0}\right) \Gamma^2 d\Omega$$

In this case, a diffuse source, the brightness (and electric field) are not angle dependent, so we can integrate easily.

$$\int d(V_{oc}^2) = \left (\frac{\lambda^2 }{4\pi} \frac{4 R_r}{Z_0} \Gamma^2 \right ) B Z_0\int D(\Omega) d\Omega$$

Simplifying
\begin{equation}\label{eq:vos_squared_complete}
V_{oc}^2 = \left (\frac{R_r \lambda^2 }{\pi} \Gamma^2 \right ) \int B D(\Omega) d\Omega
\end{equation}

Over the entire diffuse sky, the integral of the brightness is simply the flux divided by $4\pi$. Similarly, the directivity term when integrated becomes $4\pi$. This gives  
\begin{equation}
\int B D(\Omega) d\Omega = \frac{S}{4\pi} 4\pi
\end{equation}
\begin{equation}
\int B D(\Omega) d\Omega = S
\end{equation}
% ****
% Not 100\% sure about this part:
% $$D = \frac{4 \pi}{\Omega_a} $$
% [Stutzman Eq. 2-144]
% [Kraus88 Eq. 2-8-4]


% $$ S = B \int d\Omega = B 4\pi$$
% $$ \int B(r) D(r) d\Omega = \int S/4\pi D(r) d\Omega $$
% $$= S/4\pi 4\pi = S $$


% *****

Substituting this result into Eq.~\ref{eq:vos_squared_complete}
\begin{equation}
V_{oc}^2 = \left (\frac{R_r \lambda^2 }{\pi} \Gamma^2 \right ) S
\end{equation}

The final flux to voltage conversion term comes from dividing both sides by the flux to give
\begin{equation}\label{eq:flux_to_voltage_conversion}
\frac{V_{oc}^2}{S} = \frac{R_r \lambda^2 }{\pi} \Gamma^2
\end{equation}
